Robust Parameter Identifiability Analysis via Column Subset Selection

We advocate a numerically reliable and accurate approach for practical parameter identifiability analysis: Applying column subset selection (CSS) to the sensitivity matrix, instead of computing an eigenvalue decomposition of the Fischer information matrix. Identifiability analysis via CSS has three advantages: (i) It quantifies reliability of the subsets of parameters selected as identifiable and unidentifiable. (ii) It establishes criteria for comparing the accuracy of different algorithms. (iii) The implementations are numerically more accurate and reliable than eigenvalue methods applied to the Fischer matrix, yet without an increase in computational cost. The effectiveness of the CSS methods is illustrated with extensive numerical experiments on sensitivity matrices from six physical models, as well as on adversarial synthetic matrices. Among the CSS methods, we recommend an implementation based on the strong rank-revealing QR algorithm because of its rigorous accuracy guarantees for both identifiable and non-identifiable parameters.

==> aux.tex <==
More generally, let $\vx\in\real^p$ with $\|\vx\|_2=1$ and $\|\mchi\vx\|_2=\epsilon$ for 
some $\epsilon>0$. Let $\mP$ be a permutation that moves a magnitude-largest 
element of $\vx$ to the bottom, $|(\mP^T\vx)_p|=\|\vx\|_{\infty}$.
If $\mchi\mP=\mq\mr$ is a QR decomposition (\ref{e_qr}) of $\mchi\mP$, then 
the trailing diagonal element of~$\mr$ satisfies
\begin{align*}
\sigma_p\leq |r_{pp}|\leq \sqrt{p}\,\epsilon.
\end{align*}

If $\vv$
is a right singular vector of a matrix $\mb\in\real^{m\times m}$ 
corresponding to a smallest 
singular value $\sigma_m(\mb)$, then one can construct
 a permutation matrix $\mP$ 
so that a QR decomposition of $\mb\mP$ reveals $\sigma_m$ in
the trailing diagonal element of $\mb$, up to a factor $\sqrt{m}$.


Start a matrix that collects the permuted singular vectors,
$\mw^{(1)}=(\widetilde{\mP}^{(1)})^T\vv^{(1)}\in\real^p$.
It satisfies 
\begin{align*}
\|\mw^{(1)}\|_2=1, \qquad |\mw^{(1)}_p|\geq 1/\sqrt{p}, \qquad
|\mw^{(1)}_j|\leq |\mw^{(1)}_p|, \quad 1\leq j\leq p-1,
\end{align*}
and 
\begin{align*}
\mchi\mP^{(1)}\mw^{(1)}&=\mchi\mP^{(0)}\widetilde{\mP}^{(1)}
(\widetilde{\mP}^{(1)})^T\vv^{(1)}=\mchi\mP^{(0)}\vv^{(1)}=\mq^{(0)}\mr^{(0)}\vv^{(1)}\\
&=\mq^{(0)}\mr^{(1)}_{11}\vv^{(1)}=\sigma_p\mq^{(0)}\vu^{(1)}.
\end{align*}
Augment the matrix that collects the permuted singular vectors,
\begin{align*}
\mw^{(i+1)}=\begin{bmatrix}(\widetilde{P}^{(i+1)})^T&\vzero \\ \vzero &\mi_i\end{bmatrix}
\begin{bmatrix}\begin{bmatrix}\vv^{(i+1)} \\ \vzero_i\end{bmatrix} & \mw^{(i)}
\end{bmatrix}\in\real^{p\times (i+1)}
\end{align*}
The first column satisfies
\begin{align*}
\|\mw^{(i+1)}\ve_1\|_2=1, \qquad |\mw^{(i+1)}_{\ell 1}|\geq 1/\sqrt{\ell}, \qquad
|\mw^{(i+1)}_{\ell 1}|\leq |\mw^{(i+1)}_{j 1}|, \quad 1\leq j\leq \ell-1,
\end{align*}
and (\ref{e_PCAc}) implies
\begin{align*}
\mchi\mP^{(i+1)}\mw^{(i+1)}\ve_1&=\mchi\mP^{(i)}\widetilde{\mP}^{(i+1)}
(\widetilde{\mP}^{(i+1)})^T\begin{bmatrix}\vv^{(i+1)}\\\vzero_i\end{bmatrix}
=\mchi\mP^{(i)}\begin{bmatrix}\vv^{(i+1)}\\ \vzero_i\end{bmatrix}\\
&=\mq^{(i)}\mr^{(i)}\begin{bmatrix}\vv^{(i+1)}\\ \vzero_i\end{bmatrix}
=\mq^{(i)}\begin{bmatrix}\mr_{11}^{(i)} &\mr^{(i)}_{12}\\ \vzero & \mr^{(i)}_{22}
\end{bmatrix}
\begin{bmatrix}\vv^{(i+1)}\\ \vzero_i\end{bmatrix}\\
&=\mq^{(i)}\begin{bmatrix}\mr_{11}^{(i)} \vv^{(i+1)}\\ \vzero_i\end{bmatrix}
=\sigma_{\ell}(\mr_{11}^{(i)})\,\mq^{(i)} \begin{bmatrix} \vv^{(i+1)}\\ \vzero_i\end{bmatrix}
\end{align*}

